ChartBench: A Benchmark for Complex Visual Reasoning in Charts

Multimodal Large Language Models (MLLMs) have shown impressive capabilities in image understanding and generation. However, current benchmarks fail to accurately evaluate the chart comprehension of MLLMs due to limited chart types and inappropriate metrics. To address this, we propose ChartBench, a comprehensive benchmark designed to assess chart comprehension and data reliability through complex visual reasoning. ChartBench includes 42 categories, 66.6k charts, and 600k question-answer pairs. Notably, many charts lack data point annotations, which requires MLLMs to derive values similar to human understanding by leveraging inherent chart elements such as color, legends, and coordinate systems. We also design an enhanced evaluation metric, Acc+, to evaluate MLLMs without extensive manual or costly LLM-based evaluations. Furthermore, we propose two baselines based on the chain of thought and supervised fine-tuning to improve model performance on unannotated charts. Extensive experimental evaluations of 18 open-sourced and 3 proprietary MLLMs reveal their limitations in chart comprehension and offer valuable insights for further research. Code and dataset are publicly available at https://chartbench.github.io.

==> figures/texs/fig_CoT.tex <==
\begin{figure}[t]
    \centering
    \begin{overpic}[width=\linewidth, grid=False]{figures/figs/different_cot.pdf}
    \put(7,-2){\scriptsize (a) Base}
    \put(32,-2){\scriptsize (b) Fixed CoT}
    \put(58,-2){\scriptsize (c) Self CoT}
    \put(85,-2){\scriptsize (d) GPT CoT}
    \end{overpic}
    \vspace{-5pt}
    \caption{Illustration of different Chain of Thought. (a) No CoT. (b) All charts utilize the same CoT template that we provide. (c) The CoT for each chart is generated by its own LLM given the prompted question. (d) The CoT for each chart is generated by GPT given the prompted question.}
    \vspace{-15pt}
    \label{fig_CoT}
\end{figure}




==> figures/texs/fig_chart_detail.tex <==
\begin{figure}
  \centering
  \begin{subfigure}[b]{0.44\linewidth}
    \includegraphics[width=\linewidth]{figures/figs/chart_type_distribution.pdf}
    \caption{Major chart types distribution in ChartBench.}
    \label{fig_chart_type_distribution}
  \end{subfigure}
  % \vspace{-5pt}
  \hspace{5pt}
  \begin{subfigure}[b]{0.365\linewidth}
    \includegraphics[width=\linewidth]{figures/figs/chart_wi_wo_anno.pdf}
    \caption{With/without annotations chart distribution.}
    \label{fig_chart_wi_wo_anno}
  \end{subfigure}
  % \vspace{-5pt}
  \caption{Detailed chart distribution of ChartBench.}
  \vspace{-5pt}
  \label{fig_chart_detail}
\end{figure}

==> figures/texs/fig_resolution.tex <==
\begin{figure}[t]
  \centering
  \begin{overpic}[width=0.9\linewidth, grid=False]{figures/figs/resolution.pdf}
  \end{overpic}
  \caption{The zero-shot \textit{Acc+} (\%) w.r.t. query chart resolution.}
  \vspace{-10pt}
  \label{fig_resolution}
\end{figure}


==> section/check_list.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section ?.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Sec.~\ref{sec_discussion}.} 
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Appendix~\ref{apdx_sec_ethical}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{Our research performed in the paper accords with the ethics review guidelines in every aspect.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{The paper is more likely experimental, not theoretical.}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{The paper is more likely experimental, not theoretical.}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Appendix~\ref{sec_apdx_settings}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{A part of the experiments is evaluated several times.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix~\ref{sec_apdx_settings}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{See Appendix~\ref{apdx_sec_ethical}.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerYes{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tables/minipage/minipage_anno_cot.tex <==
\begin{table}[h]
    \begin{minipage}{0.48\textwidth}
        \centering
        \caption{The \textit{Acc+} (\%) performance w.r.t. data annotations. \textit{w/i} and \textit{w/o} indicate chart with and without annotations, respectively.}
        \resizebox{\linewidth}{!}{
        \setlength{\tabcolsep}{10pt}
        \begin{tabular}{@{}lcccc@{}}
        \toprule
        \multicolumn{1}{c|}{Models}             & \textit{w/i}    & \textit{w/o}    & \multicolumn{1}{c|}{$\Delta$}  & \textit{Acc+}  \\ \midrule
        \multicolumn{5}{c}{\cellcolor{tablered}Open source MLLMs}                                                       \\ 
        \multicolumn{1}{l|}{VisualGLM~\cite{glm}}          & 7.22  & 2.83  & \multicolumn{1}{r|}{\good{+4.39$\uparrow$}}   & 3.79  \\
        \multicolumn{1}{l|}{Shikra~\cite{shikra}}             & 4.17  & 9.22  & \multicolumn{1}{r|}{\bad{-5.05$\downarrow$}} & 8.11  \\
        \multicolumn{1}{l|}{InstructBLIP~\cite{InstructBLIP}}       & 14.28 & 11.98 & \multicolumn{1}{r|}{\good{+2.30$\uparrow$}}   & 12.49 \\
        \multicolumn{1}{l|}{CogVLM~\cite{cogvlm}}             & 17.67 & 12.08 & \multicolumn{1}{r|}{\good{+5.59$\uparrow$}}   & 13.30 \\
        \multicolumn{1}{l|}{Internlm-Xcomposer~\cite{internlm-xcomposer}} & 11.94 & 16.48 & \multicolumn{1}{r|}{\bad{-4.54$\downarrow$}} & 15.49 \\
        \multicolumn{1}{l|}{SPHINX~\cite{sphinx}}             & 23.22 & 16.39 & \multicolumn{1}{r|}{\good{+6.83$\uparrow$}}   & 17.89 \\
        \multicolumn{1}{l|}{ChartLlama~\cite{Chartllama}}         & 21.83 & 13.08 & \multicolumn{1}{r|}{\good{+8.75$\uparrow$}}   & 19.06 \\
        \multicolumn{1}{l|}{BLIP2~\cite{BLIP2}}              & 28.94 & 17.80 & \multicolumn{1}{r|}{\good{+11.14$\uparrow$}}  & 20.24 \\
        \multicolumn{1}{l|}{MiniGPT-v2~\cite{Minigptv2}}         & 23.83 & 23.47 & \multicolumn{1}{r|}{\good{+0.36$\uparrow$}}   & 23.55 \\
        \multicolumn{1}{l|}{LLaVA-v1.5~\cite{Improvedllava}}         & 29.72 & 25.45 & \multicolumn{1}{r|}{\good{+4.27$\uparrow$}}   & 26.39 \\
        \multicolumn{1}{l|}{mPLUG-owl-bloomz~\cite{Mplug}}   & 28.67 & 26.25 & \multicolumn{1}{r|}{\good{+2.42$\uparrow$}}   & 26.78 \\
        \multicolumn{1}{l|}{Qwen-VL-Chat~\cite{qwen-vl}}       & 40.67 & 24.67 & \multicolumn{1}{r|}{\good{\textbf{+16.00$\uparrow$}}}  & 28.18 \\ \midrule
        \multicolumn{5}{c}{\cellcolor{tablered}Closed source MLLMs}                                                         \\ 
        \multicolumn{1}{l|}{ERNIE~\cite{wenxin}}              & 51.11 & 45.78 & \multicolumn{1}{r|}{\good{+5.33$\uparrow$}}   & 46.95 \\
        \multicolumn{1}{l|}{GPT-4V~\cite{GPT4}}              & 78.89 & 47.50 & \multicolumn{1}{r|}{\textbf{\good{+31.39$\uparrow$}}}  & 54.39 \\ \bottomrule
        \end{tabular}
        }
        \label{tab_data_anno}
    \end{minipage}
    \hfill
    \begin{minipage}{0.48\textwidth}
        \centering
        \caption{Model performance with zero-shot and ChartCoT. \textit{w/i} and \textit{w/o} indicate chart with and without annotations, respectively.}
        \resizebox{\linewidth}{!}{
        \begin{tabular}{@{}cc|ccc|ccc@{}}
        \toprule
        \multicolumn{2}{c|}{\multirow{2}{*}{Metric}} & \multicolumn{3}{c|}{MiniGPT-v2~\cite{Minigptv2}} & \multicolumn{3}{c}{Qwen-VL-Chat~\cite{qwen-vl}} \\ \cmidrule(l){3-8} 
        \multicolumn{2}{c|}{} & Base & CoT & $\Delta$ & Base & CoT & $\Delta$ \\ \midrule
        \multicolumn{1}{c|}{\multirow{7}{*}{\textit{Acc+}}} & CR & 29.02 & 36.76 & \good{+7.74$\uparrow$} & 52.54 & 64.54 & \good{+12.00$\uparrow$} \\
        \multicolumn{1}{c|}{} & VE & 22.29 & 29.22 & \good{+6.93$\uparrow$} & 10.78 & 15.85 & \good{+5.07$\uparrow$} \\
        \multicolumn{1}{c|}{} & VC & 24.59 & 25.14 & \good{+0.55$\uparrow$} & 27.46 & 28.44 & \good{+0.98$\uparrow$} \\
        \multicolumn{1}{c|}{} & GC & 18.29 & 26.37 & \good{+8.08$\uparrow$} & 21.95 & 29.22 & \good{+7.27$\uparrow$} \\
        \multicolumn{1}{c|}{} & All & 23.55 & 29.37 & \good{+5.82$\uparrow$} & 28.18 & 34.51 & \good{+6.33$\uparrow$} \\
        \multicolumn{1}{c|}{} & \cellcolor{tablered}\textit{w/i} & 23.47 & 29.77 & \good{+6.30$\uparrow$} & 40.67 & 48.89 & \good{+8.22$\uparrow$} \\
        \multicolumn{1}{c|}{} & \cellcolor{tablered}\textit{w/o} & 23.83 & 29.26 & \good{+5.43$\uparrow$} & 24.67 & 30.47 & \good{+5.80$\uparrow$} \\ \midrule
        \multicolumn{1}{c|}{\multirow{7}{*}{\textit{CoR}}} & CR & 49.03 & 43.11 & \good{5.92$\downarrow$} & 41.90 & 31.66 & \good{10.24$\downarrow$} \\
        \multicolumn{1}{c|}{} & VE & 55.41 & 52.27 & \good{3.14$\downarrow$} & 85.03 & 78.24 & \good{6.79$\downarrow$} \\
        \multicolumn{1}{c|}{} & VC & 53.70 & 51.72 & \good{1.98$\downarrow$} & 62.83 & 61.86 & \good{0.97$\downarrow$} \\
        \multicolumn{1}{c|}{} & GC & 62.10 & 55.12 & \good{6.98$\downarrow$} & 74.78 & 66.73 & \good{8.05$\downarrow$} \\
        \multicolumn{1}{c|}{} & All & 55.06 & 50.55 & \good{4.51$\downarrow$} & 66.13 & 59.63 & \good{6.50$\downarrow$} \\
        \multicolumn{1}{c|}{} & \cellcolor{tablered}\textit{w/i} & 55.73 & 51.28 & \good{4.45$\downarrow$} & 69.67 & 64.02 & \good{5.65$\downarrow$} \\
        \multicolumn{1}{c|}{} & \cellcolor{tablered}\textit{w/o} & 52.67 & 50.32 & \good{2.35$\downarrow$} & 53.56 & 44.00 & \good{9.56$\downarrow$} \\ \bottomrule
        \end{tabular}
        }
        \label{tab_chartcot}
    \end{minipage}
\end{table}




==> tables/minipage/minipage_chart_task_acc_cor.tex <==
\begin{table}[h]
    \begin{minipage}{0.48\textwidth}
        \centering
        \caption{The zero-shot \textit{Acc+} (\%) performance w.r.t. chart tasks. We report the results of the best-performing prompt for each MLLM.}
        \resizebox{\linewidth}{!}{
        \begin{tabular}{@{}lccccc@{}}
        \toprule
        \multicolumn{1}{c|}{\multirow{2}{*}{Models}} & \multicolumn{4}{c|}{Task Type}                     & \multirow{2}{*}{\textit{Acc+}} \\ \cmidrule(lr){2-5}
        \multicolumn{1}{c|}{}                        & CR    & VE    & VC    & \multicolumn{1}{c|}{GC}    &                       \\ \midrule
        \multicolumn{6}{c}{\cellcolor{tablered}Open source MLLMs}                                                                                     \\
        \multicolumn{1}{l|}{VisualGLM~\cite{glm}}               & 15.17 & 0.00  & 0.00  & \multicolumn{1}{c|}{0.00}  & 3.79                  \\
        \multicolumn{1}{l|}{Shikra~\cite{shikra}}                  & 2.15  & 11.90 & 10.63 & \multicolumn{1}{c|}{7.76}  & 8.11                  \\
        \multicolumn{1}{l|}{InstructBLIP~\cite{InstructBLIP}}            & 49.90 & 0.00  & 0.05  & \multicolumn{1}{c|}{0.00}  & 12.49                 \\
        \multicolumn{1}{l|}{CogVLM~\cite{cogvlm}}                  & 29.41 & 2.39  & 14.29 & \multicolumn{1}{c|}{7.12}  & 13.30                 \\
        \multicolumn{1}{l|}{Internlm-XComposer~\cite{internlm-xcomposer}}      & 42.59 & 6.98  & 2.49  & \multicolumn{1}{c|}{9.90}  & 15.49                 \\
        \multicolumn{1}{l|}{SPHINX~\cite{sphinx}}                  & 38.15 & 9.90  & 14.15 & \multicolumn{1}{c|}{9.37}  & 17.89                 \\
        \multicolumn{1}{l|}{BLIP2~\cite{BLIP2}}                   & \textbf{59.51} & 3.85  & 13.95 & \multicolumn{1}{c|}{3.66}  & 20.24                 \\
        \multicolumn{1}{l|}{ChartLlama~\cite{Chartllama}}              & 49.51 & 8.34  & 20.54 & \multicolumn{1}{c|}{10.63} & 22.26                 \\
        \multicolumn{1}{l|}{MiniGPT-v2~\cite{Minigptv2}}              & 29.02 & 22.29 & 24.59 & \multicolumn{1}{c|}{18.29} & 23.55                 \\
        \multicolumn{1}{l|}{LLaVA-v1.5~\cite{Improvedllava}}              & 46.98 & 15.90 & 26.15 & \multicolumn{1}{c|}{16.54} & 26.39                 \\
        \multicolumn{1}{l|}{mPLUG-Owl-bloomz~\cite{Mplug}}        & 32.20 & \textbf{23.02} & 25.37 & \multicolumn{1}{c|}{\textbf{26.54}} & 26.78                 \\
        \multicolumn{1}{l|}{Qwen-VL-Chat~\cite{qwen-vl}}            & 52.54 & 10.78 & \textbf{27.46} & \multicolumn{1}{c|}{21.95} & \textbf{28.18 }                \\ \midrule
        \multicolumn{6}{c}{\cellcolor{tablered}Closed source MLLMs}                                                                                   \\ 
        \multicolumn{1}{l|}{ERNIE~\cite{wenxin}}                   & 65.37 & \textbf{43.90} & 32.20 & \multicolumn{1}{c|}{\textbf{46.34}} & 46.95                 \\
        \multicolumn{1}{l|}{GPT-4V~\cite{GPT4}}                  & \textbf{96.10} & 29.27 & \textbf{47.32} & \multicolumn{1}{c|}{44.88} & \textbf{54.39 }                \\ \bottomrule
        \end{tabular}
        }
        \vspace{-10pt}
        \label{tab_result_task}
    \end{minipage}
    \hfill
    \begin{minipage}{0.48\textwidth}
        \centering
        \caption{The zero-shot \textit{CoR}(\%) performance w.r.t. chart tasks. A lower \textit{CoR} metric indicates fewer random guessing cases.}
        \resizebox{\linewidth}{!}{
        \begin{tabular}{@{}lccccc@{}}
        \toprule
        \multicolumn{1}{c|}{\multirow{2}{*}{Models}} & \multicolumn{4}{c|}{Task Type} & \multirow{2}{*}{\textit{CoR}} \\ \cmidrule(lr){2-5}
        \multicolumn{1}{c|}{} & CR & VE & VC & \multicolumn{1}{c|}{GC} &  \\ \midrule
        \multicolumn{6}{c}{\cellcolor{tablered}Open source MLLMs} \\ 
        \multicolumn{1}{l|}{VisualGLM~\cite{glm}} & 80.20 & 99.81 & 99.90 & \multicolumn{1}{c|}{99.85} & 94.94 \\
        \multicolumn{1}{l|}{Shikra~\cite{shikra}} & 94.25 & 77.56 & 83.46 & \multicolumn{1}{c|}{80.73} & 84.00 \\
        \multicolumn{1}{l|}{InstructBLIP~\cite{InstructBLIP}} & \textbf{36.05} & 100.00 & 99.80 & \multicolumn{1}{c|}{99.90} & 83.94 \\
        \multicolumn{1}{l|}{CogVLM~\cite{cogvlm}} & 69.36 & 94.88 & 80.58 & \multicolumn{1}{c|}{90.49} & 83.83 \\
        \multicolumn{1}{l|}{ChartLlama~\cite{Chartllama}} & 78.48 & 84.98 & 73.32 & \multicolumn{1}{c|}{84.68} & 80.36 \\
        \multicolumn{1}{l|}{Internlm-XComposer~\cite{internlm-xcomposer}} & 56.64 & 84.87 & 96.54 & \multicolumn{1}{c|}{77.95} & 79.00 \\
        \multicolumn{1}{l|}{BLIP2~\cite{BLIP2}} & 37.51 & 91.07 & 80.59 & \multicolumn{1}{c|}{91.66} & 75.21 \\
        \multicolumn{1}{l|}{SPHINX~\cite{sphinx}} & 51.51 & 80.98 & 77.51 & \multicolumn{1}{c|}{81.27} & 72.82 \\
        \multicolumn{1}{l|}{Qwen-VL-Chat~\cite{qwen-vl}} & 41.90 & 85.03 & 62.83 & \multicolumn{1}{c|}{74.78} & 66.13 \\
        \multicolumn{1}{l|}{mPLUG-Owl-bloomz~\cite{Mplug}} & 58.64 & 67.26 & 61.66 & \multicolumn{1}{c|}{\textbf{61.66}} & 62.30 \\
        \multicolumn{1}{l|}{LLaVA-v1.5~\cite{Improvedllava}} & 36.78 & 66.88 & 57.02 & \multicolumn{1}{c|}{67.51} & 57.05 \\
        \multicolumn{1}{l|}{MiniGPT-v2~\cite{Minigptv2}} & 49.03 & \textbf{55.41} & \textbf{53.70} & \multicolumn{1}{c|}{62.10} & \textbf{55.06} \\ \midrule
        \multicolumn{6}{c}{\cellcolor{tablered}Closed source MLLMs} \\ 
        \multicolumn{1}{l|}{ERNIE~\cite{wenxin}} & 19.03 & \textbf{45.85} & 41.47 & \multicolumn{1}{c|}{\textbf{48.29}} & 38.66 \\
        \multicolumn{1}{l|}{GPT-4V~\cite{GPT4}} & \textbf{2.93} & 64.88 & \textbf{35.61} & \multicolumn{1}{c|}{48.78} & \textbf{38.05} \\ \bottomrule
        \end{tabular}
        }
        \label{tab_CoR}
    \end{minipage}
\end{table}




==> tables/tab_CoT.tex <==
\begin{table}[t]
\centering
\caption{Model performance with zero-shot and ChartCoT. \textit{w/i} and \textit{w/o} indicate chart with and without annotations, respectively.}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}cc|ccc|ccc@{}}
\toprule
\multicolumn{2}{c|}{\multirow{2}{*}{Metric}} & \multicolumn{3}{c|}{MiniGPT-v2} & \multicolumn{3}{c}{Qwen-VL-Chat} \\ \cmidrule(l){3-8} 
\multicolumn{2}{c|}{} & Base & CoT & $\Delta$ & Base & CoT & $\Delta$ \\ \midrule
\multicolumn{1}{c|}{\multirow{7}{*}{\textit{Acc+}}} & CR & 29.02 & 36.76 & \good{+7.74$\uparrow$} & 52.54 & 64.54 & \good{+12.00$\uparrow$} \\
\multicolumn{1}{c|}{} & VE & 22.29 & 29.22 & \good{+6.93$\uparrow$} & 10.78 & 15.85 & \good{+5.07$\uparrow$} \\
\multicolumn{1}{c|}{} & VC & 24.59 & 25.14 & \good{+0.55$\uparrow$} & 27.46 & 28.44 & \good{+0.98$\uparrow$} \\
\multicolumn{1}{c|}{} & GC & 18.29 & 26.37 & \good{+8.08$\uparrow$} & 21.95 & 29.22 & \good{+7.27$\uparrow$} \\
\multicolumn{1}{c|}{} & All & 23.55 & 29.37 & \good{+5.82$\uparrow$} & 28.18 & 34.51 & \good{+6.33$\uparrow$} \\
\multicolumn{1}{c|}{} & \cellcolor{tablered}\textit{w/i} & 23.47 & 29.77 & \good{+6.30$\uparrow$} & 40.67 & 48.89 & \good{+8.22$\uparrow$} \\
\multicolumn{1}{c|}{} & \cellcolor{tablered}\textit{w/o} & 23.83 & 29.26 & \good{+5.43$\uparrow$} & 24.67 & 30.47 & \good{+5.80$\uparrow$} \\ \midrule
\multicolumn{1}{c|}{\multirow{7}{*}{\textit{CoR}}} & CR & 49.03 & 43.11 & \good{5.92$\downarrow$} & 41.90 & 31.66 & \good{10.24$\downarrow$} \\
\multicolumn{1}{c|}{} & VE & 55.41 & 52.27 & \good{3.14$\downarrow$} & 85.03 & 78.24 & \good{6.79$\downarrow$} \\
\multicolumn{1}{c|}{} & VC & 53.70 & 51.72 & \good{1.98$\downarrow$} & 62.83 & 61.86 & \good{0.97$\downarrow$} \\
\multicolumn{1}{c|}{} & GC & 62.10 & 55.12 & \good{6.98$\downarrow$} & 74.78 & 66.73 & \good{8.05$\downarrow$} \\
\multicolumn{1}{c|}{} & All & 55.06 & 50.55 & \good{4.51$\downarrow$} & 66.13 & 59.63 & \good{6.50$\downarrow$} \\
\multicolumn{1}{c|}{} & \cellcolor{tablered}\textit{w/i} & 55.73 & 51.28 & \good{4.45$\downarrow$} & 69.67 & 64.02 & \good{5.65$\downarrow$} \\
\multicolumn{1}{c|}{} & \cellcolor{tablered}\textit{w/o} & 52.67 & 50.32 & \good{2.35$\downarrow$} & 53.56 & 44.00 & \good{9.56$\downarrow$} \\ \bottomrule
\end{tabular}
}
\label{tab_chartcot}
% \vspace{-15pt}
\end{table}

==> tables/tab_acc_plus_task.tex <==
\begin{table}[t]
\centering
\caption{The zero-shot \textit{Acc+} (\%) performance w.r.t. chart tasks. We report the results of the best-performing prompt for each MLLM.}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lccccc@{}}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{Models}} & \multicolumn{4}{c|}{Task Type}                     & \multirow{2}{*}{\textit{Acc+}} \\ \cmidrule(lr){2-5}
\multicolumn{1}{c|}{}                        & CR    & VE    & VC    & \multicolumn{1}{c|}{GC}    &                       \\ \midrule
\multicolumn{6}{c}{\cellcolor{tablered}Open source MLLMs}                                                                                     \\
\multicolumn{1}{l|}{VisualGLM~\cite{glm}}               & 15.17 & 0.00  & 0.00  & \multicolumn{1}{c|}{0.00}  & 3.79                  \\
\multicolumn{1}{l|}{Shikra~\cite{shikra}}                  & 2.15  & 11.90 & 10.63 & \multicolumn{1}{c|}{7.76}  & 8.11                  \\
\multicolumn{1}{l|}{InstructBLIP~\cite{InstructBLIP}}            & 49.90 & 0.00  & 0.05  & \multicolumn{1}{c|}{0.00}  & 12.49                 \\
\multicolumn{1}{l|}{CogVLM~\cite{cogvlm}}                  & 29.41 & 2.39  & 14.29 & \multicolumn{1}{c|}{7.12}  & 13.30                 \\
\multicolumn{1}{l|}{Internlm-XComposer~\cite{internlm-xcomposer}}      & 42.59 & 6.98  & 2.49  & \multicolumn{1}{c|}{9.90}  & 15.49                 \\
\multicolumn{1}{l|}{SPHINX~\cite{sphinx}}                  & 38.15 & 9.90  & 14.15 & \multicolumn{1}{c|}{9.37}  & 17.89                 \\
\multicolumn{1}{l|}{BLIP2~\cite{BLIP2}}                   & \textbf{59.51} & 3.85  & 13.95 & \multicolumn{1}{c|}{3.66}  & 20.24                 \\
\multicolumn{1}{l|}{ChartLlama~\cite{Chartllama}}              & 49.51 & 8.34  & 20.54 & \multicolumn{1}{c|}{10.63} & 22.26                 \\
\multicolumn{1}{l|}{MiniGPT-v2~\cite{Minigptv2}}              & 29.02 & 22.29 & 24.59 & \multicolumn{1}{c|}{18.29} & 23.55                 \\
\multicolumn{1}{l|}{LLaVA-v1.5~\cite{Improvedllava}}              & 46.98 & 15.90 & 26.15 & \multicolumn{1}{c|}{16.54} & 26.39                 \\
\multicolumn{1}{l|}{mPLUG-Owl-bloomz~\cite{Mplug}}        & 32.20 & \textbf{23.02} & 25.37 & \multicolumn{1}{c|}{\textbf{26.54}} & 26.78                 \\
\multicolumn{1}{l|}{Qwen-VL-Chat~\cite{qwen-vl}}            & 52.54 & 10.78 & \textbf{27.46} & \multicolumn{1}{c|}{21.95} & \textbf{28.18 }                \\ \midrule
\multicolumn{6}{c}{\cellcolor{tablered}Closed source MLLMs}                                                                                   \\ 
\multicolumn{1}{l|}{ERNIE~\cite{wenxin}}                   & 65.37 & \textbf{43.90} & 32.20 & \multicolumn{1}{c|}{\textbf{46.34}} & 46.95                 \\
\multicolumn{1}{l|}{GPT-4V~\cite{GPT4}}                  & \textbf{96.10} & 29.27 & \textbf{47.32} & \multicolumn{1}{c|}{44.88} & \textbf{54.39 }                \\ \bottomrule
\end{tabular}
}
\vspace{-10pt}
\label{tab_result_task}
\end{table}

==> tables/tab_annotation.tex <==
\begin{table}[ht]
\centering
\caption{The \textit{Acc+} (\%) performance w.r.t. data annotations. \textit{w/i} and \textit{w/o} indicate chart with and without annotations, respectively.}
\resizebox{\linewidth}{!}{
\setlength{\tabcolsep}{10pt}
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{1}{c|}{Models}             & \textit{w/i}    & \textit{w/o}    & \multicolumn{1}{c|}{$\Delta$}  & \textit{Acc+}  \\ \midrule
\multicolumn{5}{c}{\cellcolor{tablered}Closed source MLLMs}                                                       \\ 
\multicolumn{1}{l|}{VisualGLM}          & 7.22  & 2.83  & \multicolumn{1}{r|}{\good{+4.39$\uparrow$}}   & 3.79  \\
\multicolumn{1}{l|}{Shikra}             & 4.17  & 9.22  & \multicolumn{1}{r|}{\bad{-5.05$\downarrow$}} & 8.11  \\
\multicolumn{1}{l|}{InstructBLIP}       & 14.28 & 11.98 & \multicolumn{1}{r|}{\good{+2.30$\uparrow$}}   & 12.49 \\
\multicolumn{1}{l|}{CogVLM}             & 17.67 & 12.08 & \multicolumn{1}{r|}{\good{+5.59$\uparrow$}}   & 13.30 \\
\multicolumn{1}{l|}{Internlm-Xcomposer} & 11.94 & 16.48 & \multicolumn{1}{r|}{\bad{-4.54$\downarrow$}} & 15.49 \\
\multicolumn{1}{l|}{SPHINX}             & 23.22 & 16.39 & \multicolumn{1}{r|}{\good{+6.83$\uparrow$}}   & 17.89 \\
\multicolumn{1}{l|}{ChartLlama}         & 21.83 & 13.08 & \multicolumn{1}{r|}{\good{+8.75$\uparrow$}}   & 19.06 \\
\multicolumn{1}{l|}{BLIP2}              & 28.94 & 17.80 & \multicolumn{1}{r|}{\good{+11.14$\uparrow$}}  & 20.24 \\
\multicolumn{1}{l|}{MiniGPT-v2}         & 23.83 & 23.47 & \multicolumn{1}{r|}{\good{+0.36$\uparrow$}}   & 23.55 \\
\multicolumn{1}{l|}{LLaVA-v1.5}         & 29.72 & 25.45 & \multicolumn{1}{r|}{\good{+4.27$\uparrow$}}   & 26.39 \\
\multicolumn{1}{l|}{mPLUG-owl-bloomz}   & 28.67 & 26.25 & \multicolumn{1}{r|}{\good{+2.42$\uparrow$}}   & 26.78 \\
\multicolumn{1}{l|}{Qwen-VL-Chat}       & 40.67 & 24.67 & \multicolumn{1}{r|}{\good{\textbf{+16.00$\uparrow$}}}  & 28.18 \\ \midrule
\multicolumn{5}{c}{\cellcolor{tablered}Open source MLLMs}                                                         \\ 
\multicolumn{1}{l|}{ERNIE}              & 51.11 & 45.78 & \multicolumn{1}{r|}{\good{+5.33$\uparrow$}}   & 46.95 \\
\multicolumn{1}{l|}{GPT-4V}              & 78.89 & 47.50 & \multicolumn{1}{r|}{\textbf{\good{+31.39$\uparrow$}}}  & 54.39 \\ \bottomrule
\end{tabular}
}
\label{tab_data_anno}
\vspace{-10pt}
\end{table}

==> tables/tab_leaderboard_anno_and_chartqa.tex <==
\begin{table}[t!]
% \centering
\begin{minipage}[t]{0.7\textwidth}
    \centering
    \begin{minipage}[t]{0.32\textwidth}
    \vspace{0pt}
    \centering
    \setlength\tabcolsep{4.0pt}
    \resizebox{1\linewidth}{!}{
        \begin{tabular}{c|l|c}
        \textbf{No.} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{Accuracy} \\
        \Xhline{1.0pt}
        \rowcolor{red!26}\textbf{1} & \textbf{\red{ChartLlama}} & \textbf{72.31}\\
        \rowcolor{red!21}\textbf{2} & \textbf{Qwen-VL-Chat} & \textbf{54.61}\\
        \rowcolor{red!16}\textbf{3} &  \textbf{CogVLM} & \textbf{38.90}\\
        \rowcolor{red!11}\textbf{4} & \textbf{LLaVA-v1.5} & \textbf{29.93} \\
        \rowcolor{red!6}\textbf{5} & \textbf{SPHINX} & \textbf{27.43} \\
        6 & MiniGPT-v2 & 25.44 \\
        7 & VisualGLM & 24.94 \\
        8 & Internlm-XComposer & 24.69 \\
        9 & InstructBLIP & 23.44 \\
        10 & Shikra & 19.70 \\
        11 & mPLUG-Owl-bloomz & 17.96 \\
        12 & BLIP2 & 11.72 \\
        \end{tabular}
    }
    % \vspace{-0.3cm}
    \subcaption{\textit{Line Chart}}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\textwidth}
    \vspace{0pt}
    \centering
    \setlength\tabcolsep{4.0pt}
    \resizebox{1\linewidth}{!}{
        \begin{tabular}{c|l|c}
        \textbf{No.} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{Accuracy} \\
        \Xhline{1.0pt}
        \rowcolor{blue!26}\textbf{1} & \textbf{\red{ChartLlama}} & \textbf{77.01}\\
        \rowcolor{blue!21}\textbf{2} & \textbf{Qwen-VL-Chat} & \textbf{60.72}\\
        \rowcolor{blue!16}\textbf{3} &  \textbf{CogVLM} & \textbf{29.68}\\
        \rowcolor{blue!11}\textbf{4} & \textbf{LLaVA-v1.5} & \textbf{16.29} \\
        \rowcolor{blue!6}\textbf{5} & \textbf{SPHINX} & \textbf{14.06} \\
        6 & MiniGPT-v2 & 13.23 \\
        7 & Internlm-XComposer & 10.90 \\
        8 & VisualGLM & 10.85 \\
        9 & InstructBLIP & 10.69 \\
        10 & Shikra & 10.02 \\
        11 & mPLUG-Owl-bloomz & 7.78 \\
        12 & BLIP2 & 7.11 \\
        \end{tabular}
    }
    % \vspace{-0.3cm}
    \subcaption{\textit{Bar Chart}}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\textwidth}
    \vspace{0pt}
    \centering
    \setlength\tabcolsep{4.0pt}
    \resizebox{1\linewidth}{!}{
        \begin{tabular}{c|l|c}
        \textbf{No.} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{Accuracy} \\
        \Xhline{1.0pt}
        \rowcolor{green!26}\textbf{1} & \textbf{\red{ChartLlama}} & \textbf{69.77}\\
        \rowcolor{green!21}\textbf{2} & \textbf{Qwen-VL-Chat} & \textbf{47.67}\\
        \rowcolor{green!16}\textbf{3} &  \textbf{CogVLM} & \textbf{33.14}\\
        \rowcolor{green!16}\textbf{4} & \textbf{LLaVA-v1.5} & \textbf{16.28} \\
        \rowcolor{green!16}\textbf{5} & \textbf{SPHINX} & \textbf{15.70} \\
        6 & Shikra & 12.21 \\
        7 & MiniGPT-v2 & 11.05 \\
        8 & InstructBLIP & 10.47 \\
        9 & Internlm-XComposer & 10.47 \\
        10 & VisualGLM & 6.98 \\
        11 & mPLUG-Owl-bloomz & 6.40 \\
        12 & BLIP2 & 6.40 \\
        \end{tabular}
    }
    % \vspace{-0.3cm}
    \subcaption{\textit{Pie Chart}}
    \end{minipage}
    \vspace{0.1cm}

    \begin{minipage}[t]{0.32\textwidth}
    \vspace{0pt}
    \centering
    \setlength\tabcolsep{4.0pt}
    \resizebox{1\linewidth}{!}{
        \begin{tabular}{c|l|c}
        \textbf{No.} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{Accuracy} \\
        \Xhline{1.0pt}
        \rowcolor{yellow!26}\textbf{1} & \textbf{\red{ChartLlama}} & \textbf{58.40}\\
        \rowcolor{yellow!21}\textbf{2} & \textbf{Qwen-VL-Chat} & \textbf{42.48}\\
        \rowcolor{yellow!16}\textbf{3} &  \textbf{CogVLM} & \textbf{34.24}\\
        \rowcolor{yellow!11}\textbf{4} & \textbf{LLaVA-v1.5} & \textbf{23.20} \\
        \rowcolor{yellow!6}\textbf{5} & \textbf{SPHINX} & \textbf{21.44} \\
        6 & MiniGPT-v2 & 19.28 \\
        7 & VisualGLM & 17.76 \\
        8 & Internlm-XComposer & 16.80 \\
        9 & Shikra & 16.16 \\
        10 & InstructBLIP & 15.60 \\
        11 & mPLUG-Owl-bloomz & 12.72 \\
        12 & BLIP2 & 10.40 \\
        \end{tabular}
    }
    % \vspace{-0.3cm}
    \subcaption{\textit{Human Split}}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\textwidth}
    \vspace{0pt}
    \centering
    \setlength\tabcolsep{4.0pt}
    \resizebox{1\linewidth}{!}{
        \begin{tabular}{c|l|c}
        \textbf{No.} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{Accuracy} \\
        \Xhline{1.0pt}
        \rowcolor{orange!26}\textbf{1} & \textbf{\red{ChartLlama}} & \textbf{93.12}\\
        \rowcolor{orange!21}\textbf{2} & \textbf{Qwen-VL-Chat} & \textbf{75.20}\\
        \rowcolor{orange!16}\textbf{3} &  \textbf{CogVLM} & \textbf{28.56}\\
        \rowcolor{orange!11}\textbf{4} & \textbf{LLaVA-v1.5} & \textbf{13.76} \\
        \rowcolor{orange!6}\textbf{5} & \textbf{SPHINX} & \textbf{11.20} \\
        6 & MiniGPT-v2 & 10.80 \\
        7 & InstructBLIP & 9.84 \\
        8 & Internlm-XComposer & 9.36 \\
        9 & VisualGLM & 7.92 \\
        10 & Shikra & 7.28 \\
        11 & mPLUG-Owl-bloomz & 5.92 \\
        12 & BLIP2 & 5.20 \\
        \end{tabular}
    }
    % \vspace{-0.3cm}
    \subcaption{\textit{Augmented Split}}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\textwidth}
    \vspace{0pt}
    \centering
    \setlength\tabcolsep{4.0pt}
    \resizebox{1\linewidth}{!}{
        \begin{tabular}{c|l|c}
        \textbf{No.} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{Accuracy} \\
        \Xhline{1.0pt}
        \rowcolor{gray!26}\textbf{1} & \textbf{\red{ChartLlama}} & \textbf{75.76}\\
        \rowcolor{gray!21}\textbf{2} & \textbf{Qwen-VL-Chat} & \textbf{58.84}\\
        \rowcolor{gray!16}\textbf{3} &  \textbf{CogVLM} & \textbf{31.40}\\
        \rowcolor{gray!11}\textbf{4} & \textbf{LLaVA-v1.5} & \textbf{18.48} \\
        \rowcolor{gray!6}\textbf{5} & \textbf{SPHINX} & \textbf{16.32} \\
        6 & MiniGPT-v2 & 15.04 \\
        7 & Internlm-XComposer & 13.08 \\
        8 & VisualGLM & 12.84 \\
        9 & InstructBLIP & 12.72 \\
        10 & Shikra & 11.72 \\
        11 & mPLUG-Owl-bloomz & 9.32 \\
        12 & BLIP2 & 7.80 \\
        \end{tabular}
    }
    % \vspace{-0.3cm}
    \subcaption{\textit{Average}}
    \end{minipage}
    \caption{Leaderboards of different tasks, dataset splits and average on ChartQA. We utilize the original query in ChartQA as prompt.}
    \label{leaderboard_chartqa}
\end{minipage}

% \hspace{2mm}

\begin{minipage}{0.22\textwidth}
    \centering
    \begin{minipage}[t]{0.9\textwidth}
    \vspace{0pt}
    \centering
    \setlength\tabcolsep{4.0pt}
    \resizebox{1\linewidth}{!}{
        \begin{tabular}{c|l|c}
        \textbf{No.} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Acc+}} \\
        \Xhline{1.0pt}
        \rowcolor{red!26}\textbf{1} & \textbf{\red{GPT-4V}} & \textbf{78.89}\\
        \rowcolor{red!21}\textbf{2} & \textbf{ERNIE} & \textbf{51.11}\\
        \rowcolor{red!16}\textbf{3} &  \textbf{QWen-VL-Chat} & \textbf{40.67}\\
        \rowcolor{red!11}\textbf{4} & \textbf{LLaVA-v1.5} & \textbf{29.72} \\
        \rowcolor{red!6}\textbf{5} & \textbf{ChartLlama} & \textbf{28.94} \\
        6 & mPLUG-Owl-bloomz & 28.67 \\
        7 & MiniGPT-v2 & 23.83 \\
        8 & SPHINX & 23.22 \\
        9 & BLIP2 & 21.83 \\
        10 & CogVLM & 17.67 \\
        11 & InstructBLIP & 14.28 \\
        12 & Internlm-XComposer & 11.94 \\
        % 13 & VisualGLM & 7.22 \\
        % 14 & Shikra & 4.17 \\
        \end{tabular}
    }
    % \vspace{-0.3cm}
    \subcaption{\textit{w/i Annotations.}}
    \end{minipage}
    \\
    \vspace{0.1cm}
    \begin{minipage}[t]{0.9\textwidth}
    \vspace{0pt}
    \centering
    \setlength\tabcolsep{4.0pt}
    \resizebox{1\linewidth}{!}{
        \begin{tabular}{c|l|c}
        \textbf{No.} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Acc+}} \\
        \Xhline{1.0pt}
        \rowcolor{blue!26}\textbf{1} & \textbf{\red{GPT-4V}} & \textbf{47.95}\\
        \rowcolor{blue!21}\textbf{2} & \textbf{ERNIE} & \textbf{45.78}\\
        \rowcolor{blue!16}\textbf{3} &  \textbf{mPLUG-Owl-bloomz} & \textbf{26.25}\\
        \rowcolor{blue!11}\textbf{4} & \textbf{LLaVA-v1.5} & \textbf{25.45} \\
        \rowcolor{blue!6}\textbf{5} & \textbf{QWen-VL-Chat} & \textbf{24.67} \\
        6 & MiniGPT-v2 & 23.47 \\
        7 & ChartLlama & 17.80 \\
        8 & Internlm-XComposer & 16.48 \\
        9 & SPHINX & 16.39 \\
        10 & BLIP2 & 13.08 \\
        11 & CogVLM & 12.08 \\
        12 & InstructBLIP & 11.98 \\
        % 13 & Shikra & 9.22 \\
        % 14 & VisualGLM & 2.83 \\
        \end{tabular}
    }
    % \vspace{-0.3cm}
    \subcaption{\textit{w/o Annotations.}}
    \end{minipage}
    \caption{Leaderboards w.r.t. data annotations of \textit{Acc+} (\%) performance on ChartBench.}
    \label{leaderboard_anno}
\end{minipage}

\end{table}

==> tables/tab_leaderboard_chartqa.tex <==
\begin{table*}[tp]
\centering
\begin{minipage}[t]{0.22\textwidth}
    \vspace{0pt}
    \centering
    \setlength\tabcolsep{4.0pt}
    \resizebox{1\linewidth}{!}{
        \begin{tabular}{c|l|c}
        \textbf{No.} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{Accuracy} \\
        \Xhline{1.0pt}
        \rowcolor{red!26}\textbf{1} & \textbf{\red{ChartLlama}} & \textbf{72.31}\\
        \rowcolor{red!21}\textbf{2} & \textbf{Qwen-VL-Chat} & \textbf{54.61}\\
        \rowcolor{red!16}\textbf{3} &  \textbf{CogVLM} & \textbf{38.90}\\
        \rowcolor{red!11}\textbf{4} & \textbf{LLaVA-v1.5} & \textbf{29.93} \\
        \rowcolor{red!6}\textbf{5} & \textbf{SPHINX} & \textbf{27.43} \\
        6 & MiniGPT-v2 & 25.44 \\
        7 & VisualGLM & 24.94 \\
        8 & Internlm-XComposer & 24.69 \\
        9 & InstructBLIP & 23.44 \\
        10 & Shikra & 19.70 \\
        11 & mPLUG-Owl-bloomz & 17.96 \\
        12 & BLIP2 & 11.72 \\
        \end{tabular}
    }
    % \vspace{-0.3cm}
    \subcaption{\textit{Line Chart}}
\end{minipage}
\hfill
\begin{minipage}[t]{0.22\textwidth}
    \vspace{0pt}
    \centering
    \setlength\tabcolsep{4.0pt}
    \resizebox{1\linewidth}{!}{
        \begin{tabular}{c|l|c}
        \textbf{No.} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{Accuracy} \\
        \Xhline{1.0pt}
        \rowcolor{blue!26}\textbf{1} & \textbf{\red{ChartLlama}} & \textbf{77.01}\\
        \rowcolor{blue!21}\textbf{2} & \textbf{Qwen-VL-Chat} & \textbf{60.72}\\
        \rowcolor{blue!16}\textbf{3} &  \textbf{CogVLM} & \textbf{29.68}\\
        \rowcolor{blue!11}\textbf{4} & \textbf{LLaVA-v1.5} & \textbf{16.29} \\
        \rowcolor{blue!6}\textbf{5} & \textbf{SPHINX} & \textbf{14.06} \\
        6 & MiniGPT-v2 & 13.23 \\
        7 & Internlm-XComposer & 10.90 \\
        8 & VisualGLM & 10.85 \\
        9 & InstructBLIP & 10.69 \\
        10 & Shikra & 10.02 \\
        11 & mPLUG-Owl-bloomz & 7.78 \\
        12 & BLIP2 & 7.11 \\
        \end{tabular}
    }
    % \vspace{-0.3cm}
    \subcaption{\textit{Bar Chart}}
\end{minipage}
\hfill
\begin{minipage}[t]{0.22\textwidth}
    \vspace{0pt}
    \centering
    \setlength\tabcolsep{4.0pt}
    \resizebox{1\linewidth}{!}{
        \begin{tabular}{c|l|c}
        \textbf{No.} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{Accuracy} \\
        \Xhline{1.0pt}
        \rowcolor{green!26}\textbf{1} & \textbf{\red{ChartLlama}} & \textbf{69.77}\\
        \rowcolor{green!21}\textbf{2} & \textbf{Qwen-VL-Chat} & \textbf{47.67}\\
        \rowcolor{green!16}\textbf{3} &  \textbf{CogVLM} & \textbf{33.14}\\
        \rowcolor{green!16}\textbf{4} & \textbf{LLaVA-v1.5} & \textbf{16.28} \\
        \rowcolor{green!16}\textbf{5} & \textbf{SPHINX} & \textbf{15.70} \\
        6 & Shikra & 12.21 \\
        7 & MiniGPT-v2 & 11.05 \\
        8 & InstructBLIP & 10.47 \\
        9 & Internlm-XComposer & 10.47 \\
        10 & VisualGLM & 6.98 \\
        11 & mPLUG-Owl-bloomz & 6.40 \\
        12 & BLIP2 & 6.40 \\
        \end{tabular}
    }
    % \vspace{-0.3cm}
    \subcaption{\textit{Pie Chart}}
\end{minipage}
\vspace{0.1cm}

\begin{minipage}[t]{0.22\textwidth}
    \vspace{0pt}
    \centering
    \setlength\tabcolsep{4.0pt}
    \resizebox{1\linewidth}{!}{
        \begin{tabular}{c|l|c}
        \textbf{No.} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{Accuracy} \\
        \Xhline{1.0pt}
        \rowcolor{yellow!26}\textbf{1} & \textbf{\red{ChartLlama}} & \textbf{58.40}\\
        \rowcolor{yellow!21}\textbf{2} & \textbf{Qwen-VL-Chat} & \textbf{42.48}\\
        \rowcolor{yellow!16}\textbf{3} &  \textbf{CogVLM} & \textbf{34.24}\\
        \rowcolor{yellow!11}\textbf{4} & \textbf{LLaVA-v1.5} & \textbf{23.20} \\
        \rowcolor{yellow!6}\textbf{5} & \textbf{SPHINX} & \textbf{21.44} \\
        6 & MiniGPT-v2 & 19.28 \\
        7 & VisualGLM & 17.76 \\
        8 & Internlm-XComposer & 16.80 \\
        9 & Shikra & 16.16 \\
        10 & InstructBLIP & 15.60 \\
        11 & mPLUG-Owl-bloomz & 12.72 \\
        12 & BLIP2 & 10.40 \\
        \end{tabular}
    }
    % \vspace{-0.3cm}
    \subcaption{\textit{Human Split}}
\end{minipage}
\hfill
\begin{minipage}[t]{0.22\textwidth}
    \vspace{0pt}
    \centering
    \setlength\tabcolsep{4.0pt}
    \resizebox{1\linewidth}{!}{
        \begin{tabular}{c|l|c}
        \textbf{No.} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{Accuracy} \\
        \Xhline{1.0pt}
        \rowcolor{orange!26}\textbf{1} & \textbf{\red{ChartLlama}} & \textbf{93.12}\\
        \rowcolor{orange!21}\textbf{2} & \textbf{Qwen-VL-Chat} & \textbf{75.20}\\
        \rowcolor{orange!16}\textbf{3} &  \textbf{CogVLM} & \textbf{28.56}\\
        \rowcolor{orange!11}\textbf{4} & \textbf{LLaVA-v1.5} & \textbf{13.76} \\
        \rowcolor{orange!6}\textbf{5} & \textbf{SPHINX} & \textbf{11.20} \\
        6 & MiniGPT-v2 & 10.80 \\
        7 & InstructBLIP & 9.84 \\
        8 & Internlm-XComposer & 9.36 \\
        9 & VisualGLM & 7.92 \\
        10 & Shikra & 7.28 \\
        11 & mPLUG-Owl-bloomz & 5.92 \\
        12 & BLIP2 & 5.20 \\
        \end{tabular}
    }
    % \vspace{-0.3cm}
    \subcaption{\textit{Augmented Split}}
\end{minipage}
\hfill
\begin{minipage}[t]{0.22\textwidth}
    \vspace{0pt}
    \centering
    \setlength\tabcolsep{4.0pt}
    \resizebox{1\linewidth}{!}{
        \begin{tabular}{c|l|c}
        \textbf{No.} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{Accuracy} \\
        \Xhline{1.0pt}
        \rowcolor{gray!26}\textbf{1} & \textbf{\red{ChartLlama}} & \textbf{75.76}\\
        \rowcolor{gray!21}\textbf{2} & \textbf{Qwen-VL-Chat} & \textbf{58.84}\\
        \rowcolor{gray!16}\textbf{3} &  \textbf{CogVLM} & \textbf{31.40}\\
        \rowcolor{gray!11}\textbf{4} & \textbf{LLaVA-v1.5} & \textbf{18.48} \\
        \rowcolor{gray!6}\textbf{5} & \textbf{SPHINX} & \textbf{16.32} \\
        6 & MiniGPT-v2 & 15.04 \\
        7 & Internlm-XComposer & 13.08 \\
        8 & VisualGLM & 12.84 \\
        9 & InstructBLIP & 12.72 \\
        10 & Shikra & 11.72 \\
        11 & mPLUG-Owl-bloomz & 9.32 \\
        12 & BLIP2 & 7.80 \\
        \end{tabular}
    }
    % \vspace{-0.3cm}
    \subcaption{\textit{Average}}
\end{minipage}
\caption{Leaderboards of different tasks, dataset splits and average on ChartQA. We utilize the original query in ChartQA as prompt.}
\label{leaderboard_chartqa}
\end{table*}

==> tables/tab_mistake.tex <==
\begin{table}[t]
\centering
\caption{The zero-shot \textit{CoR}(\%) performance w.r.t. chart tasks. A lower \textit{CoR} metric indicates fewer random guessing cases.}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lccccc@{}}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{Models}} & \multicolumn{4}{c|}{Task Type} & \multirow{2}{*}{\textit{CoR}} \\ \cmidrule(lr){2-5}
\multicolumn{1}{c|}{} & CR & VE & VC & \multicolumn{1}{c|}{GC} &  \\ \midrule
\multicolumn{6}{c}{\cellcolor{tablered}Open source MLLMs} \\ 
\multicolumn{1}{l|}{VisualGLM} & 80.20 & 99.81 & 99.90 & \multicolumn{1}{c|}{99.85} & 94.94 \\
\multicolumn{1}{l|}{Shikra} & 94.25 & 77.56 & 83.46 & \multicolumn{1}{c|}{80.73} & 84.00 \\
\multicolumn{1}{l|}{InstructBLIP} & \textbf{36.05} & 100.00 & 99.80 & \multicolumn{1}{c|}{99.90} & 83.94 \\
\multicolumn{1}{l|}{CogVLM} & 69.36 & 94.88 & 80.58 & \multicolumn{1}{c|}{90.49} & 83.83 \\
\multicolumn{1}{l|}{ChartLlama} & 78.48 & 84.98 & 73.32 & \multicolumn{1}{c|}{84.68} & 80.36 \\
\multicolumn{1}{l|}{Internlm-XComposer} & 56.64 & 84.87 & 96.54 & \multicolumn{1}{c|}{77.95} & 79.00 \\
\multicolumn{1}{l|}{BLIP2} & 37.51 & 91.07 & 80.59 & \multicolumn{1}{c|}{91.66} & 75.21 \\
\multicolumn{1}{l|}{SPHINX} & 51.51 & 80.98 & 77.51 & \multicolumn{1}{c|}{81.27} & 72.82 \\
\multicolumn{1}{l|}{Qwen-VL-Chat} & 41.90 & 85.03 & 62.83 & \multicolumn{1}{c|}{74.78} & 66.13 \\
\multicolumn{1}{l|}{mPLUG-Owl-bloomz} & 58.64 & 67.26 & 61.66 & \multicolumn{1}{c|}{\textbf{61.66}} & 62.30 \\
\multicolumn{1}{l|}{LLaVA-v1.5} & 36.78 & 66.88 & 57.02 & \multicolumn{1}{c|}{67.51} & 57.05 \\
\multicolumn{1}{l|}{MiniGPT-v2} & 49.03 & \textbf{55.41} & \textbf{53.70} & \multicolumn{1}{c|}{62.10} & \textbf{55.06} \\ \midrule
\multicolumn{6}{c}{\cellcolor{tablered}Closed source MLLMs} \\ 
\multicolumn{1}{l|}{ERNIE} & 19.03 & \textbf{45.85} & 41.47 & \multicolumn{1}{c|}{\textbf{48.29}} & 38.66 \\
\multicolumn{1}{l|}{GPT-4V} & \textbf{2.93} & 64.88 & \textbf{35.61} & \multicolumn{1}{c|}{48.78} & \textbf{38.05} \\ \bottomrule
\end{tabular}
}
\label{tab_CoR}
\vspace{-10pt}
\end{table}
